Sparse estimation of parameter support sets for generalized vector autoregressions by resampling and model aggregation

The central problem we address in this work is estimation of the parameter support set S, the set of indices corresponding to nonzero parameters, in the context of a sparse parametric likelihood model for discrete multivariate time series. We develop an algorithm that performs the estimation by aggregating support sets obtained by applying the LASSO to data subsamples. Our approach is to identify several candidate models and estimate S by selecting common parameters, thus "aggregating" candidate models. While our method is broadly applicable to any selection problem, we focus on the generalized vector autoregressive (GVAR) model class, and particularly the Poisson case, emphasizing applications in network recovery from discrete multivariate time series. We propose benchmark methods based on the LASSO, develop simulation strategies for GVAR processes, and present empirical results demonstrating the superior performance of our method. Additionally, we present an application estimating ecological interaction networks from paleoclimatology data.

==> figures/parameter-estimates.tex <==
% latex table generated in R 4.4.1 by xtable 1.8-4 package
% Sun Oct 20 16:20:30 2024
\begin{table}[ht]
\centering
\caption{Parameter estimates computed on data from Pleistocene epoch according to each of the three methods, displayed according to origin and terminus in the directed graph of $\hat{A}$. Parameters estimated as exactly zero by all three methods are excluded.}
\begin{tabular}{ll|lll}
  \hline
Origin & Terminus & Naive & Benchmark & Aggregation \\ 
  \hline
actinocyclus curvatulus & actinoptychus spp & 0.004 &  &  \\ 
  actinocyclus curvatulus & coscinodiscus spp & -0.002 &  &  \\ 
  actinocyclus curvatulus & roperia tesselata & -0.033 &  &  \\ 
  actinocyclus octonarius & actinocyclus octonarius & 0.017 &  &  \\ 
  actinocyclus octonarius & actinoptychus spp & 0.015 &  &  \\ 
  actinocyclus octonarius & coscinodiscus spp & -0.006 &  &  \\ 
  actinoptychus spp & actinocyclus curvatulus & 0.021 &  &  \\ 
  actinoptychus spp & actinocyclus octonarius & 0.011 &  &  \\ 
  actinoptychus spp & azpeitia nodulifer & -0.005 &  &  \\ 
  actinoptychus spp & cyclotella spp & -0.002 &  &  \\ 
  azpeitia nodulifer & actinocyclus curvatulus & -0.012 & -0.025 & -0.025 \\ 
  azpeitia nodulifer & actinoptychus spp & -0.016 & -0.017 & -0.017 \\ 
  azpeitia nodulifer & azpeitia nodulifer & 0.011 & 0.016 & 0.016 \\ 
  azpeitia nodulifer & cyclotella spp & 0.005 &  &  \\ 
  azpeitia nodulifer & roperia tesselata & -0.059 & -0.067 &  \\ 
  coscinodiscus spp & actinocyclus curvatulus & -0.018 &  &  \\ 
  coscinodiscus spp & actinocyclus octonarius & -0.027 &  &  \\ 
  coscinodiscus spp & actinoptychus spp & -0.012 &  &  \\ 
  coscinodiscus spp & azpeitia nodulifer & 0.011 &  &  \\ 
  coscinodiscus spp & coscinodiscus spp & 0.002 &  &  \\ 
  coscinodiscus spp & roperia tesselata & 0.010 &  &  \\ 
  cyclotella spp & actinocyclus octonarius & -0.029 &  &  \\ 
  cyclotella spp & cyclotella spp & 0.004 &  &  \\ 
  roperia tesselata & actinocyclus curvatulus & 0.021 &  &  \\ 
  roperia tesselata & actinoptychus spp & 0.011 &  &  \\ 
  roperia tesselata & azpeitia nodulifer & -0.056 &  &  \\ 
  roperia tesselata & coscinodiscus spp & 0.008 &  &  \\ 
  roperia tesselata & roperia tesselata & 0.034 &  &  \\ 
   \hline
\end{tabular}
\end{table}


% latex table generated in R 4.4.1 by xtable 1.8-4 package
% Sun Oct 20 16:24:12 2024
\begin{table}[ht]
\centering
\caption{Parameter estimates computed on data from Holocene epoch according to each of the three methods, displayed according to origin and terminus in the directed graph of $\hat{A}$. Parameters estimated as exactly zero by all three methods are excluded.}
\begin{tabular}{ll|lll}
  \hline
Origin & Terminus & Naive & Benchmark & Aggregation \\ 
  \hline
actinocyclus curvatulus & actinocyclus curvatulus & 0.008 &  &  \\ 
  actinocyclus curvatulus & roperia tesselata & -0.004 &  &  \\ 
  actinocyclus octonarius & cyclotella spp & -0.002 &  &  \\ 
  actinocyclus octonarius & roperia tesselata & 0.005 &  &  \\ 
  actinoptychus spp & actinocyclus octonarius & -0.004 &  &  \\ 
  actinoptychus spp & actinoptychus spp & 0.007 & 0.006 & 0.006 \\ 
  actinoptychus spp & azpeitia nodulifer & $|$a$|$$<$0.001 &  &  \\ 
  actinoptychus spp & cyclotella spp & -0.002 &  &  \\ 
  azpeitia nodulifer & actinocyclus octonarius & -0.006 &  &  \\ 
  azpeitia nodulifer & azpeitia nodulifer & 0.045 & 0.057 & 0.061 \\ 
  azpeitia nodulifer & coscinodiscus spp & -0.003 &  &  \\ 
  azpeitia nodulifer & cyclotella spp & 0.006 &  &  \\ 
  azpeitia nodulifer & roperia tesselata & -0.006 &  &  \\ 
  coscinodiscus spp & actinoptychus spp & -0.001 &  &  \\ 
  coscinodiscus spp & azpeitia nodulifer & -0.026 &  &  \\ 
  coscinodiscus spp & cyclotella spp & -0.003 &  &  \\ 
  coscinodiscus spp & roperia tesselata & 0.029 & 0.036 & 0.024 \\ 
  cyclotella spp & actinocyclus curvatulus & $|$a$|$$<$0.001 &  &  \\ 
  cyclotella spp & coscinodiscus spp & -0.006 & -0.007 & -0.008 \\ 
  cyclotella spp & cyclotella spp & 0.025 & 0.027 & 0.027 \\ 
  cyclotella spp & roperia tesselata & -0.008 & -0.006 &  \\ 
  roperia tesselata & actinocyclus curvatulus & -0.002 &  &  \\ 
  roperia tesselata & actinocyclus octonarius & 0.003 &  &  \\ 
  roperia tesselata & actinoptychus spp & 0.002 &  &  \\ 
  roperia tesselata & azpeitia nodulifer & -0.013 & -0.010 &  \\ 
  roperia tesselata & coscinodiscus spp & $|$a$|$$<$0.001 & 0.001 &  \\ 
  roperia tesselata & roperia tesselata & 0.010 & 0.012 &  \\ 
  roperia tesselata & stephanopyxis spp & -0.013 &  &  \\ 
   \hline
\end{tabular}
\end{table}

